Accelerating MPI Collectives with Process-in-Process-based Multi-object Techniques

In the exascale computing era, optimizing MPI collective performance in high-performance computing (HPC) applications is critical. Current algorithms face performance degradation due to system call overhead, page faults, or data-copy latency, affecting HPC applications' efficiency and scalability. To address these issues, we propose PiP-MColl, a Process-in-Process-based Multi-object Inter-process MPI Collective design that maximizes small message MPI collective performance at scale. PiP-MColl features efficient multiple sender and receiver collective algorithms and leverages Process-in-Process shared memory techniques to eliminate unnecessary system call, page fault overhead, and extra data copy, improving intra- and inter-node message rate and throughput. Our design also boosts performance for larger messages, resulting in comprehensive improvement for various message sizes. Experimental results show that PiP-MColl outperforms popular MPI libraries, including OpenMPI, MVAPICH2, and Intel MPI, by up to 4.6X for MPI collectives like MPI_Scatter and MPI_Allgather.

==> Makefile <==
#
# $Id: Makefile 279 2008-01-27 16:19:38Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

HEADER = ACMmain
PICS = picture
BIB = bib
TEX = tex

TARGETS: $(HEADER).pdf
.PHONY: all clean $(HEADER).pdf

tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
pic_files = $(shell find $(PICS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
	)

$(HEADER).pdf: $(HEADER).tex $(tex_files) $(bib_files) $(pic_files)
	@if test "`which rubber`" != "" ; then \
		TEXMFOUTPUT=`pwd` rubber -c 'setlist arguments -shell-escape' --unsafe -d -f $(HEADER) ; \
	else \
		pdflatex -shell-escape $(HEADER) | tee latex.out ; \
		if grep -q 'Citation.*undefined' latex.out; then \
			bibtex $(HEADER); \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex -shell-escape $(HEADER) | tee latex.out; \
		done ; \
		rm -f latex.out ; \
	fi

clean:
	@if test "`which rubber`" != "" ; then \
		rubber -c 'setlist arguments -shell-escape' -d --clean $(HEADER) ; \
	else \
		find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
			\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
			\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
			\( -name '*.toc' -print \) -or \( -name '*.fdb_latexmk' -print \) -or \
			\( -name '*.fls' -print \) -or \( -name '*.synctex.gz' -print \) | xargs rm -f; \
		rm -f $(HEADER).dvi $(HEADER).log $(HEADER).ps $(HEADER).pdf $(HEADER).out \
			_region_* TAGS ; \
	fi

